Duplex Sequence-to-Sequence Learning for Reversible Machine Translation

Sequence-to-sequence learning naturally has two directions. How to effectively utilize supervision signals from both directions? Existing approaches either require two separate models, or a multitask-learned model but with inferior performance. In this paper, we propose REDER (Reversible Duplex Transformer), a parameter-efficient model and apply it to machine translation. Either end of REDER can simultaneously input and output a distinct language. Thus REDER enables reversible machine translation by simply flipping the input and output ends. Experiments verify that REDER achieves the first success of reversible machine translation, which helps outperform its multitask-trained baselines by up to 1.3 BLEU.

==> 025prelim.tex <==



\textbf{The standard sequence-to-sequence models}.
\textit{Sequence-to-sequence} (seq2seq) tasks~\citep{sutskever2014sequence} such as machine translation~\cite{bahdanau2014neural} typically adopt neural \textit{encoder-decoder} models which aim to approximate the mapping function $f^{\rightarrow}_{\theta_{\rx\ry}}$ from source domain $\mathcal{X}$ to target domain $\mathcal{Y}$ ($\mathcal{X} \mapsto \mathcal{Y}$). 
The encoder-decoder neural networks can be analogous to a simplex communication system in source-to-target direction (\Figref{fig:models} (a)): the encoder reads the source sequence from the source side and the decoder generates the target sequence from the target side.
Reverse travel from the target to the source side is not allowed in such simplex models.
% We therefore refer its computational model as \textit{simplex} seq2seq model. 
In this paper, we focus on the most widely-used simplex model, the Transformer model~\cite{vaswani2017attention}. 
A Transformer-based model reads a source sequence ${\mathbf{x}}=\langle x_1, \dots, x_{|\mathbf{x}|}\rangle$ and transforms to encoded representations $\mathbf{H}$ by its encoder.
% \jjx{encoded and encoder seem to duplicate; it would be better to add a whole description about transformer before diving into details. For example: and transforms to hidden representations $\mathbf{H}$ by its encoder. Given $\mathbf{H}$, the decoder is then responsible for generating a target sequence. To be specific, .... }.
The encoder is composed of $L$ stacked Transformer layers, each of which contains a self attention (\textsc{San}) and feed-forward networks (\textsc{Ffn}): 
\begin{align}
    % \mathbf{H}_{l} &= \mathcal{M}^{\rm enc}_{l}(\mathbf{H}_{l-1}) \\
    \Tilde{\mathbf{H}}_{l} &= \mathbf{H}_{l-1} + \textsc{San}(\mathbf{H}_{l-1}),  & 
    \mathbf{H}_{l} &= \Tilde{\mathbf{H}}_{l} + \textsc{Ffn}(\Tilde{\mathbf{H}}_{l}),  \nonumber
\end{align}
where $\mathbf{H}_{0} = \bm{x}$ is the sequence of word embeddings of $\mathbf{x}$, and for ease of understanding, we package layer normalization~\cite{ba2016layer} inside residual blocks and omit its formulation details.
Given the final encoded representation $\mathbf{H}_{L}$,
% \jjx{here cross attention network is strange, needs more clarifications. "with an additional cross attention network" can be deleted and CAN can be introduced after the following equation} 
the representations $\mathbf{Z}_{l}$  of each decoder layer are computed as:
\begin{align}
    % \mathbf{H}_{l} &= \mathcal{M}^{\rm enc}_{l}(\mathbf{H}_{l-1}) \\
    \Bar{\mathbf{Z}}_{l} &= \mathbf{Z}_{l-1} + \textsc{San}(\mathbf{Z}_{l-1}), ~~~
     \Tilde{\mathbf{Z}}_{l} = \Bar{\mathbf{Z}}_{l} + \textsc{Can}(\Bar{\mathbf{Z}}_{l}, \mathbf{H}_{L}), \nonumber \\
    \mathbf{Z}_{l} & = \Tilde{\mathbf{Z}}_{l} + \textsc{Ffn}(\Tilde{\mathbf{Z}}_{l}), 
    ~~~~\text{where~~}  \mathbf{Z}_{0} = \bm{\mathtt{shift\_right}(y)},
    \nonumber
\end{align}
% \jjx{the equation seems strange. Each line with one equation? zzx: space limits}
where \textsc{Can} denotes the cross attention network that can fetch time-dependent context from the encoder, $\bm{y}$ is the sequence of target word embeddings. 
Finally, it generates the corresponding target sequence ${\mathbf{y}}=\langle y_1, \dots, y_{|\mathbf{y}|}\rangle$ autoregressively by $p(y_i|\mathbf{y}_{<i}, \mathbf{x} ; \theta_{\rx\ry}) = \mathrm{softmax}(\bm{y}_i^\top \mathbf{Z}_{L,i})$ (see \citet{vaswani2017attention} for more details). 
% \jjx{need transitional sentences from structure description to objective descriptions. For example, given $(\mathbf{x},\mathbf{y})$, the target of Transformer network is to maximize the conditional probability.... }
% Given parallel examples $(\mathbf{x},\mathbf{y})$, the objective of Transformer is to maximize the conditional probability: $ \mathrm{max}_{\mathcal{M}_{\rx\ry}}~p(\mathbf{y}|\mathbf{x}) = \prod_i p(y_i|\mathbf{y}_{<i}, \mathbf{x}) $ over a target sequence given a source sequence on parallel bilingual data. 
Given the same parallel data, we can also learn a reverse mapping $f^{\leftarrow}_{\theta_{\ry\rx}}$ of the target-to-source direction ($\mathcal{X} \mapsto \mathcal{Y}$) using another simplex model.

To leverage bidirectional learning signals, another possible choice is to employ multitask learning to a simplex model $f^{\rightarrow}_{\theta}$ to jointly model both directions, where both directions share the same model parameters ($\theta = \theta_{\rm xy} = \theta_{\rm yx}$) and from the same input end to the same output end.
However, such models may suffer from the challenges of the parameter interference due to the limited network capacity~\cite{arivazhagan2019massively,zhang2021share}, where encoder and decoder are required to simultaneously understand and generate different languages, and the two different directional tasks compete for the limited shared network capacity.
% e.g., the encoder and decoder are required to simultaneously understand and generate different languages, and the two different directional tasks compete for the limited shared network capacity.

% \jjx{confusing, must be separate? shared seems also makes sense. zzx: not have to be separate. But I just mean it can be learned by a separate one.}


\textbf{Duplex sequence-to-sequence models.}
% 1. Mxy Myx is approximately inverse
% 2. what if a M and M-1 shares parametrization and model both direction?
\jjx{I still do not get the motivation of duplex based on current description for the following reasons. 1. I have no idea what is structure duality. 2. Why shared encoder-decoder can not achieve this goal? 3. Which advantages do duplex models have?}
As we stated above, the standard sequence-to-sequence generation model resembles a simplex communication channel. 
Think of a scenario where one person from New York is making a phone call to another one in Berlin. 
The phone is simplex -- it only takes voice input at New York, while only outputs voice at Berlin. 
This certainly reduced the benefit of two-way communication. 
Obviously, the everyday phone has the capability of taking voice input and producing voice output at both ends and transferring the signals in both communication directions.  
In analog, it will benefit sequence generation tasks such as machine translation 
by enabling a \emph{duplex sequence-to-sequence model}. 

Informally, a sequence-to-sequence model is \emph{duplex} if it has two ends, both with sequence input and output capability, and share a same architecture to map from one sequence space to the other and vice versa. 
\begin{definition}
\label{def:duplex-seq2seq}
A sequence-to-sequence model with parameter $\theta$ is duplex if it satisfies the following:
its network has two ends: a source end and a target end; both source and target ends can take input and output sequences;
the network defines a forward mapping function $f^{\rightarrow}_\theta: V_s^* \rightarrow V_t^*$ and a reverse mapping function $f^{\leftarrow}_\theta: V_t^* \rightarrow V_s^*$, where $V_s$, $V_t$ are the vocabularies of the source and target domains $\mathcal{X}$, $\mathcal{Y}$, and $V_s^*$, $V_t^*$ are all possible sequences;
essentially, it simultaneously induces both a forward sequence generation function and its mathematical inverse by reversely executing the network,
i.e. $f^{\leftarrow}_\theta=(f^{\rightarrow}_\theta)^{-1}$ and $f^{\rightarrow}_\theta=(f^{\leftarrow}_\theta)^{-1}$.
In addition, these two functions should satisfy the following,
\begin{equation}
% %%% \vspace{-20pt}
\begin{aligned}
    \forall \mathbf{x} \in V_s^*, f^{\leftarrow}_\theta\left(f^{\rightarrow}_\theta (\mathbf{x})\right) = \mathbf{x}  \\
    \forall \mathbf{y} \in V_t^*, f^{\rightarrow}_\theta\left(f^{\leftarrow}_\theta (\mathbf{y})\right) = \mathbf{y} 
\end{aligned}
\nonumber
\end{equation}
\end{definition}
Notice that the forward function $f^{\rightarrow}_\theta$ has the same model parameter $\theta$ as the reverse function $f^{\leftarrow}_\theta$.
% Essentially, the duplex model simultaneously induces both a forward sequence generation function and its mathematical inverse, 
% i.e. $f^{\leftarrow}_\theta=(f^{\rightarrow}_\theta)^{-1}$ and $f^{\rightarrow}_\theta=(f^{\leftarrow}_\theta)^{-1}$.
This sequence generation model following this definition behaves similarly to a two-way communication channel. 

We can apply this definition on machine translation to get a reversible translation model. 
Such a reversible model will be able to take a sentence in the source language from the source end and to output a sentence in the target language to the target end. 
With the same model it will be able to generate the reverse translation by taking a sentence in the target language from the target end to the source end. 
\begin{remark}
A reversible machine translation model using duplex sequence-to-sequence is distinct from a multilingual MT model (e.g. multilingual Transformer). 
The multilingual Transformer takes input sentences in two (or more) languages only from the same end and outputs to the other end. Its output end cannot be used to receive input signals. 
\end{remark}

% \hidethis{
% We find that the forward and reverse directions of many sequence-to-sequence problems have their structural duality~\cite{he2016dual}, where both simplex models $M_{\rm yx}$ and $M_{\rm yx}$ could be approximate inverse of each other: $M_{\rm xy} = M_{\rm yx}^{-1}$.
% It is wondering that could we construct a duplex neural network $\mathcal{M}$, which is reversible and has an architectural inverse network $\mathcal{M}^{-1}$ sharing the same parameters with $\mathcal{M}$, such that $\mathcal{M}$ models the forward direction and  $\mathcal{M}^{-1}$ models the reverse direction?
% \jjx{what is structural duality? Add more clarification or examples?} 
% % Although some previous studies propose to leverage the duality to boost two separate simplex seq2seq models of the opposite directions  (see Section~\ref{sec:related}), what if a unified model that allows duplex communication ($\mathcal{X} \mapsto \mathcal{Y}$ and $\mathcal{Y} \mapsto \mathcal{X}$) between two domains and share? 
% Formally, we define a model $\mathcal{M}$ as a \textit{duplex} seq2seq model when $\mathcal{M}$ is mathematically reversible that unifies both directional modeling, i.e., $\mathcal{M}$ models source-to-target mapping, whilst it has an architectural inverse $\mathcal{M}^{-1}$ modeling the reverse mapping from target to source domain. In other word, it satisfies
% {\begin{align}
%     \mathcal{M}:~ \mathcal{X} \mapsto \mathcal{Y}~~~~~~~\mathcal{M}^{-1}:~ \mathcal{Y} \mapsto \mathcal{X}, \nonumber\\
%     \forall x \in X:~\mathcal{M}^{-1} \circ \mathcal{M}(x) = x, \nonumber\\
%     \forall y \in Y:~\mathcal{M} \circ \mathcal{M}^{-1}(y) = y. \nonumber
% \end{align}}%
% In such a way, a duplex model allows a double-channel  \jjx{double-channel is confusing, dual channel or revertible channel?} information flow to move back and forth, helping model better capture structural duality of the given seq2seq problem. Meanwhile, duplex seq2seq models jointly optimize the two directional probabilities: $ \mathrm{max}_{\mathcal{M}}~p(\mathbf{y}|\mathbf{x}) + p(\mathbf{x}|\mathbf{y})$.
% }


















% \section{Sequence-to-Sequence Modeling: from Simplex Models to Duplex Models}
% \textbf{Sequence-to-Sequence Modeling as Simplex Communication System.}
% \textit{Sequence-to-sequence} (seq2seq) tasks~\citep{sutskever2014sequence} such as machine translation~\cite{bahdanau2014neural} typically adopt \textit{encoder-decoder} models $\mathcal{M}_{\rx\ry}$ which aim to approximate the mapping from source domain $X$ to target domain $Y$ ($\mathcal{X} \mapsto \mathcal{Y}$). Such injection mapping can be analogous to a simplex communication system in source-to-target direction. We therefore refer its computational model as \textit{simplex} seq2seq model. Although there are varity of simplex seq2seq models, in this paper, we focus on the widely-used Transformer model~\cite{vaswani2017attention}. A Transformer-based model $\mathcal{M}_{\rx\ry}$ reads a source sequence ${\mathbf{x}}=\langle x_1, \dots, x_{|\mathbf{x}|}\rangle$ and transforms to encoded representations $\mathbf{H}$ by its encoder \jjx{encoded and encoder seem to duplicate; it would be better to add a whole description about transformer before diving into details. For example: and transforms to hidden representations $\mathbf{H}$ by its encoder. Given $\mathbf{H}$, the decoder is then responsible for generating a target sequence. To be specific, .... }. The encoder is composed of $L$ stacked Transformer layers, each of which contains a self attention (\textsc{San}) and feed-forward networks (\textsc{Ffn}): 
% \begin{align}
%     % \mathbf{H}_{l} &= \mathcal{M}^{\rm enc}_{l}(\mathbf{H}_{l-1}) \\
%     \Tilde{\mathbf{H}}_{l} &= \mathbf{H}_{l-1} + \textsc{San}(\mathbf{H}_{l-1}),  & 
%     \mathbf{H}_{l} &= \Tilde{\mathbf{H}}_{l} + \textsc{Ffn}(\Tilde{\mathbf{H}}_{l}),  \nonumber
% \end{align}
% where $\mathbf{H}_{0} = \bm{x}$ is the sequence of word embeddings of $\mathbf{x}$, and for ease of understanding, we package layer normalization~\cite{ba2016layer} inside residual blocks and omit its formulation details.
% Given the final encoded representation $\mathbf{H}_{L}$,
% % \jjx{here cross attention network is strange, needs more clarifications. "with an additional cross attention network" can be deleted and CAN can be introduced after the following equation} 
% the representations $\mathbf{Z}_{l}$  of each decoder layer are computed as:
% \begin{align}
%     % \mathbf{H}_{l} &= \mathcal{M}^{\rm enc}_{l}(\mathbf{H}_{l-1}) \\
%     \Bar{\mathbf{Z}}_{l} &= \mathbf{Z}_{l-1} + \textsc{San}(\mathbf{Z}_{l-1}), ~~~
%      \Tilde{\mathbf{Z}}_{l} = \Bar{\mathbf{H}}_{l} + \textsc{Can}(\Bar{\mathbf{Z}}_{l}, \mathbf{H}_{L}), \nonumber \\
%     \mathbf{Z}_{l} & = \Tilde{\mathbf{Z}}_{l} + \textsc{Ffn}(\Tilde{\mathbf{Z}}_{l}), 
%     ~~~~\text{where~~}  \mathbf{Z}_{0} = \bm{\mathtt{right\_shift}(y)},
%     \nonumber
% \end{align}
% \jjx{the equation seems strange. Each line with one equation? zzx: space limits}
% where \textsc{Can} denotes the cross attention network that fetches time-dependent context from the encoder given each decoder state as query, $\bm{y}$ is the sequence of target word embeddings. 
% Finally, it generates the corresponding target sequence ${\mathbf{y}}=\langle y_1, \dots, y_{|\mathbf{y}|}\rangle$ autoregressively \jjx{auto-regressively?} by $p(y_i|\mathbf{y}_{<i}, \mathbf{x}) = \mathrm{softmax}(\bm{y}_i^\top \mathbf{Z}_{L,i})$ (see \citet{vaswani2017attention} for more details). 
% % \jjx{need transitional sentences from structure description to objective descriptions. For example, given $(\mathbf{x},\mathbf{y})$, the target of Transformer network is to maximize the conditional probability.... }
% Given parallel examples $(\mathbf{x},\mathbf{y})$, the objective of Transformer is to maximize the conditional probability: $ \mathrm{max}_{\mathcal{M}_{\rx\ry}}~p(\mathbf{y}|\mathbf{x}) = \prod_i p(y_i|\mathbf{y}_{<i}, \mathbf{x}) $ over a target sequence given a source sequence on parallel bilingual data. 
% Likewise, given the same parallel data, we can also learn a reverse mapping $\mathcal{M}_{\ry\rx}$ of the target-to-source direction using another simplex model. \jjx{confusing, must be separate? shared seems also makes sense. zzx: not have to be separate. But I just mean it can be learned by a separate one.}


% \textbf{Duplex Sequence-to-Sequence Models.}
% \jjx{I still do not get the motivation of duplex based on current description for the following reasons. 1. I have no idea what is structure duality. 2. Why shared encoder-decoder can not achieve this goal? 3. Which avantages do duplex models have?}
% We find that the forward and reverse directions of many sequence-to-sequence problems have their structural duality~\cite{he2016dual}. \jjx{what is structural duality? Add more clarification or examples?} 
% Although some previous studies propose to leverage the duality to boost two separate simplex seq2seq models of the opposite directions  (see Section~\ref{sec:related}), what if a unified model that allows duplex communication ($\mathcal{X} \mapsto \mathcal{Y}$ and $\mathcal{Y} \mapsto \mathcal{X}$) between two domains? 
% Here, we define a model $\mathcal{M}$ as a \textit{duplex} seq2seq model when $\mathcal{M}$ is mathematically reversible that unifies both directional modeling, i.e., $\mathcal{M}$ models source-to-target mapping, whilst it has an architectural inverse $\mathcal{M}^{-1}$ modeling the reverse mapping from target to source domain. In other word, it satisfies
% {\begin{align}
%     \mathcal{M}:~ \mathcal{X} \mapsto \mathcal{Y}~~~~~~~\mathcal{M}^{-1}:~ \mathcal{Y} \mapsto \mathcal{X}, \nonumber\\
%     \forall x \in X:~\mathcal{M}^{-1} \circ \mathcal{M}(x) = x, \nonumber\\
%     \forall y \in Y:~\mathcal{M} \circ \mathcal{M}^{-1}(y) = y. \nonumber
% \end{align}}%
% In such a way, a duplex model allows a double-channel  \jjx{double-channel is confusing, dual channel or revertible channel?} information flow to move back and forth, helping model better capture structural duality of the given seq2seq problem. Meanwhile, duplex seq2seq models jointly optimize the two directional probabilities: $ \mathrm{max}_{\mathcal{M}}~p(\mathbf{y}|\mathbf{x}) + p(\mathbf{x}|\mathbf{y})$.

==> tables/multi.tex <==
% \begin{table}[t]
% \centering
%     % \small
%     \caption{Comparisons between \method and \textit{multilingual} simplex approaches, which shares encoder and decoder for both translation directions, on WMT14 \textsc{En}$\leftrightarrow$\textsc{De}. }
%     \label{tab:shared-encdec}
%     \resizebox{.48\textwidth}{!}{%
%     \begin{tabular}{lccc}
%     \toprule
%     Systems & \sc En-De & \sc De-En & $|\mathbf{\theta}|$\\
%     \midrule
%     AT (separate training) & 27.60 & 31.50 & 62M$\times$2 \\
%     AT (\textit{multilingual}, joint training) & 27.05   & 30.96 & 62M  \\
%     NAT + CTC (separate training) & 26.11 & 30.24 & 62M $\times2$  \\
%     NAT + CTC (\textit{multilingual}, joint training) & 24.03  & 28.45 & 62M  \\
%     \midrule
%     \method (\textit{multilingual}, w/ CTC) & 25.58   & 28.90 & 58M \\
%     % Agreement-baed ~\cite{Cheng:2015:arXiv} &   &  & 0.980   \\
%     \method                   & 26.70 & 30.68 & 58M \\
%     \bottomrule
%     \end{tabular}%
%     }
% %\vspace{-10pt}
% \end{table}
\begin{wraptable}[22]{r}{0.55\linewidth}
% \begin{table}[t]
\centering
    % \small
    \vspace{-17pt}
% \begin{table}[t]
% \vspace{-17pt}
\centering
    % \small
    \caption{Comparisons on bidirectional translation with simplex AT and NAT models that use \textit{multi-task} learning, on WMT14 \textsc{En}$\leftrightarrow$\textsc{De}.
    ``bidir.'' means whether models can perform bidirectional translation between two languages by itself, othewise unidirectional translation as usual.
    ``-multi'' means achieving bidirectional translation by multi-task learning via adding language-specific tokens, while
    ``-reverible'' means using reversible model, i.e., \method.
    ``GLAT+CTC'' means our re-implementation of \citet{gu2020fully}, while ``$^*$'' means results from their paper. All CTC-based models decode using beam search and AT-reranking.
    ``b'' is beam size. }
    % \zzx{todo: big model}
    \label{tab:multi}
    \resizebox{.55\textwidth}{!}{%
    \begin{tabular}{lcccc}
    \toprule
    Systems & bidir.  & $|\mathbf{\theta}|$ & \sc En-De & \sc De-En\\
    \midrule
    $[1]$ AT (b=5)  & \xmark  & 62M$\times$2 & 27.60 & \bf 31.50 \\
    $[2]$ AT (b=20) & \xmark  & 62M$\times$2 & \bf 27.65 & 31.12 \\
    $[3]$ AT-multi (b=5) & \checkmark  & 62M  & 27.05   & 30.96 \\
    \hline
    $[4]$ $^*$NAT: GLAT+CTC (b=1)  & \xmark  & $|\theta|\times1$ & $^*$27.49 & $^*$31.10 \\
    $[5]$ NAT: GLAT+CTC (b=20)  & \xmark   & 62M$\times2$     & 26.79 & 30.45\\
    $[6]$ NAT-multi: GLAT+CTC (b=20) & \checkmark & 62M$\times1$ & 25.50  & 29.49  \\
    \midrule
    $[7]$ REDER (b=20)        & \xmark  & 58M$\times2$    & 26.30   & 30.12  \\
    $[8]$ REDER-multi (b=20)  & \checkmark  & 58M$\times1$    & 25.89   & 29.32 \\
    $[9]$ REDER-reversible (b=20) & \checkmark & 58M$\times1$  &\bf 27.36 &\bf 31.10  \\
    \bottomrule
    \end{tabular}%
    }
    % \vspace{-15pt}
% \end{table}
\end{wraptable}
